Safehaul: Risk-Averse Learning for Reliable mmWave Self-Backhauling in 6G Networks

Wireless backhauling at millimeter-wave frequencies (mmWave) in static scenarios is a well-established practice in cellular networks. However, highly directional and adaptive beamforming in today's mmWave systems have opened new possibilities for self-backhauling. Tapping into this potential, 3GPP has standardized Integrated Access and Backhaul (IAB) allowing the same base station serve both access and backhaul traffic. Although much more cost-effective and flexible, resource allocation and path selection in IAB mmWave networks is a formidable task. To date, prior works have addressed this challenge through a plethora of classic optimization and learning methods, generally optimizing a Key Performance Indicator (KPI) such as throughput, latency, and fairness, and little attention has been paid to the reliability of the KPI. We propose Safehaul, a risk-averse learning-based solution for IAB mmWave networks. In addition to optimizing average performance, Safehaul ensures reliability by minimizing the losses in the tail of the performance distribution. We develop a novel simulator and show via extensive simulations that Safehaul not only reduces the latency by up to 43.2% compared to the benchmarks but also exhibits significantly more reliable performance (e.g., 71.4% less variance in achieved latency).

==> DataSet/S2/Results/drop_bar.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={IAD node Count},
xmajorgrids,
xmin=0.5, xmax=15.5,
xtick style={color=black},
xtick={2,6,10,14},
xticklabels={25,50,75,100},
y grid style={darkgray176},
ylabel={dropped Packet [\%]},
ymajorgrids,
ymin=0.121938371618494, ymax=0.189310401666795,
ytick style={color=black}
]
\addplot [blue, forget plot]
table {%
0.75 0.125923238513293
1.25 0.125923238513293
1.25 0.127813721487889
0.75 0.127813721487889
0.75 0.125923238513293
};
\addplot [blue, forget plot]
table {%
1 0.125923238513293
1 0.12500073662069
};
\addplot [blue, forget plot]
table {%
1 0.127813721487889
1 0.128748674682032
};
\addplot [blue, forget plot]
table {%
0.875 0.12500073662069
1.125 0.12500073662069
};
\addplot [blue, forget plot]
table {%
0.875 0.128748674682032
1.125 0.128748674682032
};
\addplot [blue, forget plot]
table {%
4.75 0.132352559906428
5.25 0.132352559906428
5.25 0.134546268717064
4.75 0.134546268717064
4.75 0.132352559906428
};
\addplot [blue, forget plot]
table {%
5 0.132352559906428
5 0.131251195389903
};
\addplot [blue, forget plot]
table {%
5 0.134546268717064
5 0.135621638731868
};
\addplot [blue, forget plot]
table {%
4.875 0.131251195389903
5.125 0.131251195389903
};
\addplot [blue, forget plot]
table {%
4.875 0.135621638731868
5.125 0.135621638731868
};
\addplot [blue, forget plot]
table {%
8.75 0.138755494265436
9.25 0.138755494265436
9.25 0.141257451662658
8.75 0.141257451662658
8.75 0.138755494265436
};
\addplot [blue, forget plot]
table {%
9 0.138755494265436
9 0.137501549110024
};
\addplot [blue, forget plot]
table {%
9 0.141257451662658
9 0.142499656334049
};
\addplot [blue, forget plot]
table {%
8.875 0.137501549110024
9.125 0.137501549110024
};
\addplot [blue, forget plot]
table {%
8.875 0.142499656334049
9.125 0.142499656334049
};
\addplot [blue, forget plot]
table {%
12.75 0.138610818330819
13.25 0.138610818330819
13.25 0.140773365979216
12.75 0.140773365979216
12.75 0.138610818330819
};
\addplot [blue, forget plot]
table {%
13 0.138610818330819
13 0.137500622472193
};
\addplot [blue, forget plot]
table {%
13 0.140773365979216
13 0.141873033931746
};
\addplot [blue, forget plot]
table {%
12.875 0.137500622472193
13.125 0.137500622472193
};
\addplot [blue, forget plot]
table {%
12.875 0.141873033931746
13.125 0.141873033931746
};
\addplot [orange, forget plot]
table {%
1.75 0.13939696105069
2.25 0.13939696105069
2.25 0.143159352109845
1.75 0.143159352109845
1.75 0.13939696105069
};
\addplot [orange, forget plot]
table {%
2 0.13939696105069
2 0.137502270126317
};
\addplot [orange, forget plot]
table {%
2 0.143159352109845
2 0.144998030240818
};
\addplot [orange, forget plot]
table {%
1.875 0.137502270126317
2.125 0.137502270126317
};
\addplot [orange, forget plot]
table {%
1.875 0.144998030240818
2.125 0.144998030240818
};
\addplot [orange, forget plot]
table {%
5.75 0.139811415851655
6.25 0.139811415851655
6.25 0.144441104961761
5.75 0.144441104961761
5.75 0.139811415851655
};
\addplot [orange, forget plot]
table {%
6 0.139811415851655
6 0.137500729825488
};
\addplot [orange, forget plot]
table {%
6 0.144441104961761
6 0.146874425302812
};
\addplot [orange, forget plot]
table {%
5.875 0.137500729825488
6.125 0.137500729825488
};
\addplot [orange, forget plot]
table {%
5.875 0.146874425302812
6.125 0.146874425302812
};
\addplot [orange, forget plot]
table {%
9.75 0.145695766432972
10.25 0.145695766432972
10.25 0.149747868461544
9.75 0.149747868461544
9.75 0.145695766432972
};
\addplot [orange, forget plot]
table {%
10 0.145695766432972
10 0.143750668306776
};
\addplot [orange, forget plot]
table {%
10 0.149747868461544
10 0.151873545395546
};
\addplot [orange, forget plot]
table {%
9.875 0.143750668306776
10.125 0.143750668306776
};
\addplot [orange, forget plot]
table {%
9.875 0.151873545395546
10.125 0.151873545395546
};
\addplot [orange, forget plot]
table {%
13.75 0.15237628386635
14.25 0.15237628386635
14.25 0.157006301834858
13.75 0.157006301834858
13.75 0.15237628386635
};
\addplot [orange, forget plot]
table {%
14 0.15237628386635
14 0.150002577586071
};
\addplot [orange, forget plot]
table {%
14 0.157006301834858
14 0.159369095087912
};
\addplot [orange, forget plot]
table {%
13.875 0.150002577586071
14.125 0.150002577586071
};
\addplot [orange, forget plot]
table {%
13.875 0.159369095087912
14.125 0.159369095087912
};
\addplot [green, forget plot]
table {%
2.75 0.146408448309495
3.25 0.146408448309495
3.25 0.15176016951412
2.75 0.15176016951412
2.75 0.146408448309495
};
\addplot [green, forget plot]
table {%
3 0.146408448309495
3 0.143750816508208
};
\addplot [green, forget plot]
table {%
3 0.15176016951412
3 0.154371542584549
};
\addplot [green, forget plot]
table {%
2.875 0.143750816508208
3.125 0.143750816508208
};
\addplot [green, forget plot]
table {%
2.875 0.154371542584549
3.125 0.154371542584549
};
\addplot [green, forget plot]
table {%
6.75 0.159675899821842
7.25 0.159675899821842
7.25 0.166562081552306
6.75 0.166562081552306
6.75 0.159675899821842
};
\addplot [green, forget plot]
table {%
7 0.159675899821842
7 0.15625353660732
};
\addplot [green, forget plot]
table {%
7 0.166562081552306
7 0.169995967296067
};
\addplot [green, forget plot]
table {%
6.875 0.15625353660732
7.125 0.15625353660732
};
\addplot [green, forget plot]
table {%
6.875 0.169995967296067
7.125 0.169995967296067
};
\addplot [green, forget plot]
table {%
10.75 0.172225157900409
11.25 0.172225157900409
11.25 0.178992411750008
10.75 0.178992411750008
10.75 0.172225157900409
};
\addplot [green, forget plot]
table {%
11 0.172225157900409
11 0.168752848724049
};
\addplot [green, forget plot]
table {%
11 0.178992411750008
11 0.182499478997582
};
\addplot [green, forget plot]
table {%
10.875 0.168752848724049
11.125 0.168752848724049
};
\addplot [green, forget plot]
table {%
10.875 0.182499478997582
11.125 0.182499478997582
};
\addplot [green, forget plot]
table {%
14.75 0.173133112388196
15.25 0.173133112388196
15.25 0.181792518176571
14.75 0.181792518176571
14.75 0.173133112388196
};
\addplot [green, forget plot]
table {%
15 0.173133112388196
15 0.168757921816806
};
\addplot [green, forget plot]
table {%
15 0.181792518176571
15 0.186248036664599
};
\addplot [green, forget plot]
table {%
14.875 0.168757921816806
15.125 0.168757921816806
};
\addplot [green, forget plot]
table {%
14.875 0.186248036664599
15.125 0.186248036664599
};
\addplot [blue, forget plot]
table {%
0.75 0.126859683567204
1.25 0.126859683567204
};
\addplot [blue, forget plot]
table {%
4.75 0.13350611159282
5.25 0.13350611159282
};
\addplot [blue, forget plot]
table {%
8.75 0.14001864109094
9.25 0.14001864109094
};
\addplot [blue, forget plot]
table {%
12.75 0.139675116740499
13.25 0.139675116740499
};
\addplot [orange, forget plot]
table {%
1.75 0.141288736105202
2.25 0.141288736105202
};
\addplot [orange, forget plot]
table {%
5.75 0.142051538528095
6.25 0.142051538528095
};
\addplot [orange, forget plot]
table {%
9.75 0.147746846470132
10.25 0.147746846470132
};
\addplot [orange, forget plot]
table {%
13.75 0.154642461314132
14.25 0.154642461314132
};
\addplot [green, forget plot]
table {%
2.75 0.149113705404077
3.25 0.149113705404077
};
\addplot [green, forget plot]
table {%
6.75 0.163091913412969
7.25 0.163091913412969
};
\addplot [green, forget plot]
table {%
10.75 0.175647737320021
11.25 0.175647737320021
};
\addplot [green, forget plot]
table {%
14.75 0.177479658703792
15.25 0.177479658703792
};
\end{axis}

\end{tikzpicture}


==> DataSet/S2/Results/lat_bar.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={IAD node Count},
xmajorgrids,
xmin=0.5, xmax=15.5,
xtick style={color=black},
xtick={2,6,10,14},
xticklabels={25,50,75,100},
y grid style={darkgray176},
ylabel={Latency [ms]},
ymajorgrids,
ymin=8.16502090392354, ymax=15.5346836239926,
ytick style={color=black}
]
\addplot [blue, forget plot]
table {%
0.75 8.65229704786355
1.25 8.65229704786355
1.25 8.95667433319176
0.75 8.95667433319176
0.75 8.65229704786355
};
\addplot [blue, forget plot]
table {%
1 8.65229704786355
1 8.5000075468954
};
\addplot [blue, forget plot]
table {%
1 8.95667433319176
1 9.09999702128807
};
\addplot [blue, forget plot]
table {%
0.875 8.5000075468954
1.125 8.5000075468954
};
\addplot [blue, forget plot]
table {%
0.875 9.09999702128807
1.125 9.09999702128807
};
\addplot [blue, forget plot]
table {%
4.75 8.67830526077259
5.25 8.67830526077259
5.25 9.02123700579657
4.75 9.02123700579657
4.75 8.67830526077259
};
\addplot [blue, forget plot]
table {%
5 8.67830526077259
5 8.50000557301759
};
\addplot [blue, forget plot]
table {%
5 9.02123700579657
5 9.19980601317135
};
\addplot [blue, forget plot]
table {%
4.875 8.50000557301759
5.125 8.50000557301759
};
\addplot [blue, forget plot]
table {%
4.875 9.19980601317135
5.125 9.19980601317135
};
\addplot [blue, forget plot]
table {%
8.75 8.80681264246049
9.25 8.80681264246049
9.25 9.20334480412724
8.75 9.20334480412724
8.75 8.80681264246049
};
\addplot [blue, forget plot]
table {%
9 8.80681264246049
9 8.60005646248143
};
\addplot [blue, forget plot]
table {%
9 9.20334480412724
9 9.39979968571825
};
\addplot [blue, forget plot]
table {%
8.875 8.60005646248143
9.125 8.60005646248143
};
\addplot [blue, forget plot]
table {%
8.875 9.39979968571825
9.125 9.39979968571825
};
\addplot [blue, forget plot]
table {%
12.75 8.76936761204118
13.25 8.76936761204118
13.25 9.12239186000401
12.75 9.12239186000401
12.75 8.76936761204118
};
\addplot [blue, forget plot]
table {%
13 8.76936761204118
13 8.60004055696618
};
\addplot [blue, forget plot]
table {%
13 9.12239186000401
13 9.29996527842924
};
\addplot [blue, forget plot]
table {%
12.875 8.60004055696618
13.125 8.60004055696618
};
\addplot [blue, forget plot]
table {%
12.875 9.29996527842924
13.125 9.29996527842924
};
\addplot [orange, forget plot]
table {%
1.75 9.70810953767677
2.25 9.70810953767677
2.25 10.2939490143131
1.75 10.2939490143131
1.75 9.70810953767677
};
\addplot [orange, forget plot]
table {%
2 9.70810953767677
2 9.40033719572499
};
\addplot [orange, forget plot]
table {%
2 10.2939490143131
2 10.5994127901223
};
\addplot [orange, forget plot]
table {%
1.875 9.40033719572499
2.125 9.40033719572499
};
\addplot [orange, forget plot]
table {%
1.875 10.5994127901223
2.125 10.5994127901223
};
\addplot [orange, forget plot]
table {%
5.75 9.86763699638187
6.25 9.86763699638187
6.25 10.627143707908
5.75 10.627143707908
5.75 9.86763699638187
};
\addplot [orange, forget plot]
table {%
6 9.86763699638187
6 9.50000757101752
};
\addplot [orange, forget plot]
table {%
6 10.627143707908
6 10.9998525341853
};
\addplot [orange, forget plot]
table {%
5.875 9.50000757101752
6.125 9.50000757101752
};
\addplot [orange, forget plot]
table {%
5.875 10.9998525341853
6.125 10.9998525341853
};
\addplot [orange, forget plot]
table {%
9.75 9.82095031962965
10.25 9.82095031962965
10.25 10.4771734462256
9.75 10.4771734462256
9.75 9.82095031962965
};
\addplot [orange, forget plot]
table {%
10 9.82095031962965
10 9.50001336851422
};
\addplot [orange, forget plot]
table {%
10 10.4771734462256
10 10.7998151269759
};
\addplot [orange, forget plot]
table {%
9.875 9.50001336851422
10.125 9.50001336851422
};
\addplot [orange, forget plot]
table {%
9.875 10.7998151269759
10.125 10.7998151269759
};
\addplot [orange, forget plot]
table {%
13.75 9.98097172769283
14.25 9.98097172769283
14.25 10.7401351246374
13.75 10.7401351246374
13.75 9.98097172769283
};
\addplot [orange, forget plot]
table {%
14 9.98097172769283
14 9.6001440864509
};
\addplot [orange, forget plot]
table {%
14 10.7401351246374
14 11.0999984523762
};
\addplot [orange, forget plot]
table {%
13.875 9.6001440864509
14.125 9.6001440864509
};
\addplot [orange, forget plot]
table {%
13.875 11.0999984523762
14.125 11.0999984523762
};
\addplot [green, forget plot]
table {%
2.75 11.4195999259503
3.25 11.4195999259503
3.25 12.2789237861294
2.75 12.2789237861294
2.75 11.4195999259503
};
\addplot [green, forget plot]
table {%
3 11.4195999259503
3 11.0000217424949
};
\addplot [green, forget plot]
table {%
3 12.2789237861294
3 12.6989298319525
};
\addplot [green, forget plot]
table {%
2.875 11.0000217424949
3.125 11.0000217424949
};
\addplot [green, forget plot]
table {%
2.875 12.6989298319525
3.125 12.6989298319525
};
\addplot [green, forget plot]
table {%
6.75 12.6643473610552
7.25 12.6643473610552
7.25 13.7449515673722
6.75 13.7449515673722
6.75 12.6643473610552
};
\addplot [green, forget plot]
table {%
7 12.6643473610552
7 12.1004455016793
};
\addplot [green, forget plot]
table {%
7 13.7449515673722
7 14.2998916470452
};
\addplot [green, forget plot]
table {%
6.875 12.1004455016793
7.125 12.1004455016793
};
\addplot [green, forget plot]
table {%
6.875 14.2998916470452
7.125 14.2998916470452
};
\addplot [green, forget plot]
table {%
10.75 12.7653330338063
11.25 12.7653330338063
11.25 13.8413192724657
10.75 13.8413192724657
10.75 12.7653330338063
};
\addplot [green, forget plot]
table {%
11 12.7653330338063
11 12.2000424559937
};
\addplot [green, forget plot]
table {%
11 13.8413192724657
11 14.398111223683
};
\addplot [green, forget plot]
table {%
10.875 12.2000424559937
11.125 12.2000424559937
};
\addplot [green, forget plot]
table {%
10.875 14.398111223683
11.125 14.398111223683
};
\addplot [green, forget plot]
table {%
14.75 13.0880022126345
15.25 13.0880022126345
15.25 14.510899638958
14.75 14.510899638958
14.75 13.0880022126345
};
\addplot [green, forget plot]
table {%
15 13.0880022126345
15 12.4001043246183
};
\addplot [green, forget plot]
table {%
15 14.510899638958
15 15.1996989548986
};
\addplot [green, forget plot]
table {%
14.875 12.4001043246183
15.125 12.4001043246183
};
\addplot [green, forget plot]
table {%
14.875 15.1996989548986
15.125 15.1996989548986
};
\addplot [blue, forget plot]
table {%
0.75 8.80196037042797
1.25 8.80196037042797
};
\addplot [blue, forget plot]
table {%
4.75 8.85159780439165
5.25 8.85159780439165
};
\addplot [blue, forget plot]
table {%
8.75 8.99847754086362
9.25 8.99847754086362
};
\addplot [blue, forget plot]
table {%
12.75 8.94655054411835
13.25 8.94655054411835
};
\addplot [orange, forget plot]
table {%
1.75 9.99604780130373
2.25 9.99604780130373
};
\addplot [orange, forget plot]
table {%
5.75 10.2396807581973
6.25 10.2396807581973
};
\addplot [orange, forget plot]
table {%
9.75 10.1480169962449
10.25 10.1480169962449
};
\addplot [orange, forget plot]
table {%
13.75 10.3513680677838
14.25 10.3513680677838
};
\addplot [green, forget plot]
table {%
2.75 11.8541396529402
3.25 11.8541396529402
};
\addplot [green, forget plot]
table {%
6.75 13.207027840317
7.25 13.207027840317
};
\addplot [green, forget plot]
table {%
10.75 13.2994330768466
11.25 13.2994330768466
};
\addplot [green, forget plot]
table {%
14.75 13.7794961535625
15.25 13.7794961535625
};
\end{axis}

\end{tikzpicture}


==> DataSet/S2/Results/thr_bar.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={IAD node Count},
xmajorgrids,
xmin=0.5, xmax=15.5,
xtick style={color=black},
xtick={2,6,10,14},
xticklabels={25,50,75,100},
y grid style={darkgray176},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=39.408022531117, ymax=40.3319166516015,
ytick style={color=black}
]
\addplot [blue, forget plot]
table {%
0.75 39.9252918179626
1.25 39.9252918179626
1.25 40.074088551841
0.75 40.074088551841
0.75 39.9252918179626
};
\addplot [blue, forget plot]
table {%
1 39.9252918179626
1 39.8500281737151
};
\addplot [blue, forget plot]
table {%
1 40.074088551841
1 40.1498419202221
};
\addplot [blue, forget plot]
table {%
0.875 39.8500281737151
1.125 39.8500281737151
};
\addplot [blue, forget plot]
table {%
0.875 40.1498419202221
1.125 40.1498419202221
};
\addplot [blue, forget plot]
table {%
4.75 39.897237658806
5.25 39.897237658806
5.25 40.0938313456619
4.75 40.0938313456619
4.75 39.897237658806
};
\addplot [blue, forget plot]
table {%
5 39.897237658806
5 39.8000137386662
};
\addplot [blue, forget plot]
table {%
5 40.0938313456619
5 40.1997289976415
};
\addplot [blue, forget plot]
table {%
4.875 39.8000137386662
5.125 39.8000137386662
};
\addplot [blue, forget plot]
table {%
4.875 40.1997289976415
5.125 40.1997289976415
};
\addplot [blue, forget plot]
table {%
8.75 39.8983895156779
9.25 39.8983895156779
9.25 40.0981165822348
8.75 40.0981165822348
8.75 39.8983895156779
};
\addplot [blue, forget plot]
table {%
9 39.8983895156779
9 39.8001010697601
};
\addplot [blue, forget plot]
table {%
9 40.0981165822348
9 40.1997432244383
};
\addplot [blue, forget plot]
table {%
8.875 39.8001010697601
9.125 39.8001010697601
};
\addplot [blue, forget plot]
table {%
8.875 40.1997432244383
9.125 40.1997432244383
};
\addplot [blue, forget plot]
table {%
12.75 39.8978319690754
13.25 39.8978319690754
13.25 40.0955732651375
12.75 40.0955732651375
12.75 39.8978319690754
};
\addplot [blue, forget plot]
table {%
13 39.8978319690754
13 39.8000265888739
};
\addplot [blue, forget plot]
table {%
13 40.0955732651375
13 40.1997225612268
};
\addplot [blue, forget plot]
table {%
12.875 39.8000265888739
13.125 39.8000265888739
};
\addplot [blue, forget plot]
table {%
12.875 40.1997225612268
13.125 40.1997225612268
};
\addplot [orange, forget plot]
table {%
1.75 39.8969567033845
2.25 39.8969567033845
2.25 40.0992664809246
1.75 40.0992664809246
1.75 39.8969567033845
};
\addplot [orange, forget plot]
table {%
2 39.8969567033845
2 39.8000147679785
};
\addplot [orange, forget plot]
table {%
2 40.0992664809246
2 40.1997584200529
};
\addplot [orange, forget plot]
table {%
1.875 39.8000147679785
2.125 39.8000147679785
};
\addplot [orange, forget plot]
table {%
1.875 40.1997584200529
2.125 40.1997584200529
};
\addplot [orange, forget plot]
table {%
5.75 39.8663738097715
6.25 39.8663738097715
6.25 40.1161734972342
5.75 40.1161734972342
5.75 39.8663738097715
};
\addplot [orange, forget plot]
table {%
6 39.8663738097715
6 39.7400920227709
};
\addplot [orange, forget plot]
table {%
6 40.1161734972342
6 40.2397003488065
};
\addplot [orange, forget plot]
table {%
5.875 39.7400920227709
6.125 39.7400920227709
};
\addplot [orange, forget plot]
table {%
5.875 40.2397003488065
6.125 40.2397003488065
};
\addplot [orange, forget plot]
table {%
9.75 39.8645227746652
10.25 39.8645227746652
10.25 40.1131141039718
9.75 40.1131141039718
9.75 39.8645227746652
};
\addplot [orange, forget plot]
table {%
10 39.8645227746652
10 39.7400339050036
};
\addplot [orange, forget plot]
table {%
10 40.1131141039718
10 40.2399557792171
};
\addplot [orange, forget plot]
table {%
9.875 39.7400339050036
10.125 39.7400339050036
};
\addplot [orange, forget plot]
table {%
9.875 40.2399557792171
10.125 40.2399557792171
};
\addplot [orange, forget plot]
table {%
13.75 39.8660385940681
14.25 39.8660385940681
14.25 40.1133114815996
13.75 40.1133114815996
13.75 39.8660385940681
};
\addplot [orange, forget plot]
table {%
14 39.8660385940681
14 39.7400335843719
};
\addplot [orange, forget plot]
table {%
14 40.1133114815996
14 40.2399646354461
};
\addplot [orange, forget plot]
table {%
13.875 39.7400335843719
14.125 39.7400335843719
};
\addplot [orange, forget plot]
table {%
13.875 40.2399646354461
14.125 40.2399646354461
};
\addplot [green, forget plot]
table {%
2.75 39.8381464108376
3.25 39.8381464108376
3.25 40.141539788974
2.75 40.141539788974
2.75 39.8381464108376
};
\addplot [green, forget plot]
table {%
3 39.8381464108376
3 39.6903657651656
};
\addplot [green, forget plot]
table {%
3 40.141539788974
3 40.2899214643068
};
\addplot [green, forget plot]
table {%
2.875 39.6903657651656
3.125 39.6903657651656
};
\addplot [green, forget plot]
table {%
2.875 40.2899214643068
3.125 40.2899214643068
};
\addplot [green, forget plot]
table {%
6.75 39.7256503883573
7.25 39.7256503883573
7.25 40.0814684031683
6.75 40.0814684031683
6.75 39.7256503883573
};
\addplot [green, forget plot]
table {%
7 39.7256503883573
7 39.550136239081
};
\addplot [green, forget plot]
table {%
7 40.0814684031683
7 40.2499653088776
};
\addplot [green, forget plot]
table {%
6.875 39.550136239081
7.125 39.550136239081
};
\addplot [green, forget plot]
table {%
6.875 40.2499653088776
7.125 40.2499653088776
};
\addplot [green, forget plot]
table {%
10.75 39.6746041447089
11.25 39.6746041447089
11.25 40.0274974463341
10.75 40.0274974463341
10.75 39.6746041447089
};
\addplot [green, forget plot]
table {%
11 39.6746041447089
11 39.5000648935265
};
\addplot [green, forget plot]
table {%
11 40.0274974463341
11 40.1999346573412
};
\addplot [green, forget plot]
table {%
10.875 39.5000648935265
11.125 39.5000648935265
};
\addplot [green, forget plot]
table {%
10.875 40.1999346573412
11.125 40.1999346573412
};
\addplot [green, forget plot]
table {%
14.75 39.646925674091
15.25 39.646925674091
15.25 40.0448520970126
14.75 40.0448520970126
14.75 39.646925674091
};
\addplot [green, forget plot]
table {%
15 39.646925674091
15 39.4500177184118
};
\addplot [green, forget plot]
table {%
15 40.0448520970126
15 40.2499101738566
};
\addplot [green, forget plot]
table {%
14.875 39.4500177184118
15.125 39.4500177184118
};
\addplot [green, forget plot]
table {%
14.875 40.2499101738566
15.125 40.2499101738566
};
\addplot [blue, forget plot]
table {%
0.75 40.0001327407816
1.25 40.0001327407816
};
\addplot [blue, forget plot]
table {%
4.75 39.9919921171134
5.25 39.9919921171134
};
\addplot [blue, forget plot]
table {%
8.75 39.9971067956576
9.25 39.9971067956576
};
\addplot [blue, forget plot]
table {%
12.75 39.9963756465647
13.25 39.9963756465647
};
\addplot [orange, forget plot]
table {%
1.75 40.0008143068211
2.25 40.0008143068211
};
\addplot [orange, forget plot]
table {%
5.75 39.9906360603223
6.25 39.9906360603223
};
\addplot [orange, forget plot]
table {%
9.75 39.9896557120092
10.25 39.9896557120092
};
\addplot [orange, forget plot]
table {%
13.75 39.9881489757359
14.25 39.9881489757359
};
\addplot [green, forget plot]
table {%
2.75 39.9957695343879
3.25 39.9957695343879
};
\addplot [green, forget plot]
table {%
6.75 39.9009432030245
7.25 39.9009432030245
};
\addplot [green, forget plot]
table {%
10.75 39.8569095063117
11.25 39.8569095063117
};
\addplot [green, forget plot]
table {%
14.75 39.842170062045
15.25 39.842170062045
};
\end{axis}

\end{tikzpicture}


==> background.tex <==
% !TEX root = ./main.tex
        
\section{Risk Aversion in Multi-Armed Bandits}
%\section{Background: Risk Aversion in Multi-Armed Bandits}
\label{s:background} 

\begin{itemize}
 \item Existing literature on IAB-enabled networks focuses on the optimization of the expected value of a given cost function, e.g., throughput or latency.
\item Such approach fails to capture the variability of the function, therefore we consider risk.
\end{itemize}
